Neural networks trained with SGD learn distributions of increasing complexity

The ability of deep neural networks to generalise well even when they interpolate their training data has been explained using various "simplicity biases". These theories postulate that neural networks avoid overfitting by first learning simple functions, say a linear classifier, before learning more complex, non-linear functions. Meanwhile, data structure is also recognised as a key ingredient for good generalisation, yet its role in simplicity biases is not yet understood. Here, we show that neural networks trained using stochastic gradient descent initially classify their inputs using lower-order input statistics, like mean and covariance, and exploit higher-order statistics only later during training. We first demonstrate this distributional simplicity bias (DSB) in a solvable model of a neural network trained on synthetic data. We empirically demonstrate DSB in a range of deep convolutional networks and visual transformers trained on CIFAR10, and show that it even holds in networks pre-trained on ImageNet. We discuss the relation of DSB to other simplicity biases and consider its implications for the principle of Gaussian universality in learning.

==> content/contributions.tex <==
SG conceived the project. MR and SG analysed the perceptron model of
\cref{sec:perceptron}. SG performed the experiments of \cref{sec:cifar10}. SG
wrote the paper with input from AI and MR.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dist_inc_comp_icml"
%%% End:

